Concept-Best-Matching: Evaluating Compositionality in Emergent Communication

Artificial agents that learn to communicate in order to accomplish a given task acquire communication protocols that are typically opaque to a human. A large body of work has attempted to evaluate the emergent communication via various evaluation measures, with \emph{compositionality} featuring as a prominent desired trait. However, current evaluation procedures do not directly expose the compositionality of the emergent communication. We propose a procedure to assess the compositionality of emergent communication by finding the best-match between emerged words and natural language concepts. The best-match algorithm provides both a global score and a translation-map from emergent words to natural language concepts. To the best of our knowledge, it is the first time that such direct and interpretable mapping between emergent words and human concepts is provided.

==> top_level/chapters/90_playground.tex <==
\section{Playground}
\subsection{Background and Motivation}
\subsection{Accuracy vs Emergent Language Properties}
\subsubsection{Accuracy}
\subsubsection{TopSim}
\subsubsection{Grounded (Gold) Language and AMI}
\subsubsection{AMI drawbacks}
\subsection{The Best-Match Approach}
\subsection{Methods}
\subsubsection{Problem Definition}
\subsubsection{Bipartite Graph}
\subsubsection{The Best Match algorithm}
\subsubsection{Extending BM from words to messages}
\subsection{Experiments}
\subsubsection{experimental setup}
\textbf{\begin{itemize}
    \item The dataset (shape and thing?)
    \item The gold language
    \item The game (in short)
\end{itemize}}
\subsubsection{experiments}
\textbf{\begin{itemize}
    \item GS and QT
    \item SYM and RNN (two word lengths, and several msg lengths (for the RNN)
    \item Shape and Thing
\end{itemize}}


% \subsection{Symbolism vs Accuracy in Coordination Games}
% Good performance in coordination game is independent of high level of symbolism.
% Generally speaking, increasing the capacity of the channel increases the performance of the agents on the task, as measured by accurately differentiate targets from distractors. 
% Empirically, we observe that with large enough channel capacity, sender generates a unique message for each data sample and the receiver is able to extract the needed information from it for identifying the targets.
% One may define symbolism in may ways. For the sake of this work we seek to have one-to-one mapping between symbols and messages.

Evaluating the emerged communication is done using intrinsic (topographic similarity \cite{brighton2006understanding}, AMI \cite{mu2021emergent}) and extrinsic methods such as translation to a symbolic language.


\subsection{Aspects of the Emergent Language}
\label{sec:background-lang-aspects}
One motivation for studying the communication that emerged between artificial agents is to gain insights into the evolution of human language \citep{lazaridou2020multi}.
A large body of work is devoted to defining and quantifying natural language traits such as compositionality \citep{hupkes2020compositionality, dankers2021paradox, chaabouni2020compositionality}, systematic generalization \citep{vani2021iterated, mu2021emergent}, pragmatism \citep{andreas2016reasoning, kang2020incorporating, zaslavsky2020rate}, morphology, and more.
For that purpose, various inductive biases are sometimes proposed, which should encourage the emergence of these traits \citep{mccoy2020universal, mitchell2021challenges}.
%Presumably, such traits only emerge in rich and mature languages. For such languages to emerge, a complex, %multi-turn 
%communication within a rich environment setting should take place. Thus, utilizing simple communication games has so far led to limited success.


\paragraph{Compositionality:}
A desired property is compositionality, which enables representation of complex meanings using the meaning of parts \cite{li2019ease}. 
However, quantifying compositionality in EC is notoriously difficult \cite{lazaridou2018emergence}. 
While compositionality is considered a precondition for an emergent language to generalize at scale, recent studies found that common compositionality measures in EC like topographic similarity \cite{brighton2006understanding,lazaridou2018emergence,li2019ease} do not correlate well with success in the task \citep{chaabouni2021emergent, yao2022linking}.
Notably, most of these studies used \RefGame{} game setup.
In \citep{mu2021emergent} the authors suggest the \SetRefGame{} and \ConceptGame{} games.
In this work they use mutual information (MI) and adjusted mutual information (AMI) metrics and show that these metrics, as well as topographic similarity, correlate with successful coordination. 

%emergent languages can support generalization to novel composite meanings without conforming to notions of compositionality \yb{ref?}. 
%In addition, 


\subsection{Symbolism}
\bc{Maybe call this - latent-space decomposition }
\bc{need to decide if to change everything from symbols to concepts}
\begin{enumerate}
    \item Symbol is a discrete entity.
    Symbol has a meaning shared by many.
    Even though symbol is a discrete entity, its meaning \bc{I need to formally define it} is distributed at latent space. For example Cat is a symbol, yet there are many types of cats. The numeral $1$ is a symbol, yet there are many kinds of ones. 
    \item Symbolism is a process of transforming continuous surface in latent space into a single (discrete) point.
    \item Such transformation can happen in many points along the neural network
    \item We assume that it happen along the communication channel
    \item Thus, first requirement is that channel will be discrete
\end{enumerate}
\begin{enumerate}
    \item Discreteness is not strong enough requirement.
    \item Symbol is unique an a sense that two different messages on the channel cannot describe the same symbol.
    \item If we assume that a centroid of a latent space should be used for a symbol, then, no other point in the latent space should be used to convey the same latent space.
    \item We can use lossless compression as a measurement. If there are several messages that refer to the same symbol then we can compress them. \bc{need to formalize}  
\end{enumerate}



\bc{the bellow few important sentences needs additional formalism}
We define a symbol as a piece of (high-level) information that is common to many objects.
Thus, we associate each symbol with one of the world's FVPs.
The task of the agents during the coordination game is to discover the FVPs in the world. 
Discovering FVPs is done by assessing the messages generated by the agents during the game.
In coordination game we assumes that messages generated by the agents reveals the underlying structure of the world.
Note that agents may succeed to coordinate (namely, succeed in the coordination game) without revealing a meaningful world structure.
\bc{\textbf{The main goal of this research is to study and identify biases, algorithms and other approaches that encourage symbolism to emerge.}
We do that by directing the agents to use interpretable messages for succeeding in the coordination game.
We assume that interpretable messages are resulted from the underlying world structure that agents need to reveal in order to succeed in the game.
We define symbolism by our ability to interpret the messages generated by the agents, namely our ability to find a "simple" (parameter-less) assignment of messages to FVPs  (symbols).}



Our experimental setup involves two independent evaluation aspects: 1.evaluation of the performance on the coordination game itself and evaluation of the level of symbolism that emerged.
\subsection{The Oracle and the Symbol Mapping Function}
\bc{I need to re-write this section}
The symbol mapping function is a cornerstone in coordination games.
In these games, the direct mapping from objects to symbols in not known to the learners, nor it is explicitly available in the data.
We can thus define several symbol mapping versions:
\begin{itemize}
    \item The identity mapping. Many past works suggest a referential game in which both sender and receiver sees the same single target. \bc{need to add more. Maybe move under the Oracle mapping section}
    \item Supervised learning \bc{consider removing, this is not really part of the setting}- mapping from object to a specific symbol is provided as part of the training dataset. In such a setting the data labeler associate each object with one or more known concepts. \bc{This is different type of learning thus should not belong here - need to change}
    Specifically, agents can extract the number of unique symbols in the dataset. 
    \item Oracle mapping - in this setting there is an oracle (e.g., human) that know the mapping between object to concept.
    Still, no specific mapping is provided in the data.
    The concepts themselves are hidden from the learners.
    While targets in each data samples share the same concept(s), there is no indication regards the set of data samples that share the same concept.
    Thus, agents do not know, for example, how many different symbols exist in the world. 
    \item Random mapping \bc{consider removing and replace with sender (or agents, or teacher-student) mapping}- this mapping is the most difficult for the agents to learn from.
    In this mapping object in a single data point $ d $ need not to share the same symbol.
    With this mapping, agents expect to coordinate based on the mare fact that they see the same set of targets. \bc{need to reconsider, e.g., in the context of a single target}
    \item Sender mapping, or teacher-student. In this setting the sender choose the targets based on its world representation \bc{need to further describe and consolidate with above random mapping item}.
\end{itemize}
In this work we focus solely on oracle-based mapping function.
This is motivated by the observation that when studying the emergence of symbolic communication one cannot use symbols as part of the supervision.
Note that with oracle-mapping, supervision is provided by designating objects that share the same attribute without identifying the attribute itself. 
One may consider several levels of oracle-based mappings:
\begin{itemize}
    \item labels are from the type $ l = \{v_i^j\}^n $ where $n=1$ and $|\{v_i^j\}|$ is known to the agents (or the architecture). In words, labels are composed of a single FVP and the total number of FVPs is known and can be utilized by the agents or the architecture, e.g., in defining the channel capacity.
    \item labels are from the type $ l = \{v_i^j\}^n $ where $n=1$ but total number of FVPs is unknown
    \item labels are from the type $ l = \{v_i^j\}^n $ where $n \geq 1$. There is only an AND operator between the FVPs operands
    \item labels are any Boolean expression with $ l = \{v_i^j\}^n $ as its operands.
\end{itemize}




==> top_level/chapters/91_intro.tex <==
\section{Introduction}
A variety of communication methods can be found in nature \cite{munz2005bee, meulenbroek2022acoustic, suzuki2016semantic, holldobler1999multimodal}.
There are, however, many aspects of human language that are unique.
Emergent communication (EC), reviewed in \cite{Lazaridou2020EmergentMC,zhu2022survey}, analyzes communication developed by artificial agents that need to accomplish a coordination task.
In this multidisciplinary field of research, language learning abilities are embedded within artificial environments, and agents can use them to develop communication and interaction skills.
One motivation for studying the communication that emerged between artificial agents is to gain insights into the evolution of human language \citep{lazaridou2020multi}.
It is hoped that successful communication protocols will provide insight into the evolution and development 
%of animal communication and 
of human language.

Artificial agents acquire opaque communication protocols that does not clearly resemble human language.
As a result, most efforts focus on characterizing these differences.
Deciphering the emerging protocol may be especially pertinent as artificial agents are increasingly integrated into daily life, and possibly even communicate among themselves.
In this work we propose a rigid, fine-grained method to quantify the degree to which \emph{symbolic} communication emerges from agents' need to coordinate.

\begin{figure}[t]
\begin{center}
% \framebox[4.0in]{$\;$}
\resizebox{8cm}{!} {\includegraphics{top_level/figures/game.png}}
% \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
\end{center}
\caption{The multi-target shape differential game. Sender is inputted with a set of images, some of them are marked as targets by the Oracle. It then generate a discrete message and send it to the receiver. The receiver need to differentiate targets from distractors.}
\label{fig:shape-game}
\end{figure}

The coordination game is played by two agents, a sender \Sender{} and a receiver \Receiver{}. 
At each turn of the game, the sender \Sender{} is inputted with a set of $\sX^s$ objects , at least one of them is set by an Oracle to be the target \Target{} (see Figure \ref{fig:shape-game}). The sender sends a single message \Message{} to the receiver.
The receive \Receiver{} is inputted with a set of objects $\sX^r$, at least one of them is set by the Oracle to be the target \Target{}.
The receiver's task is to correctly identify the target(s) by deciphering the message sent by the sender and comparing it to its input objects $\sX^r$.
Importantly, while agents goal is to correctly identify the transmitted target(s), we are interested in assessing the emerged communication.

Key challenge in the field \bcr{} is the ability to assess the communication learned and used by the agents for solving a coordination task.
Communication traits are emergent properties.
Agents are not optimized towards a specific trait. Rather, agents are trained to accomplish a coordination task \bcr{}.
Consequently, there is no clear correlation between agents' ability to solve a given task and the properties of the emerging communication\bcr{}.

A large body of work is devoted to defining and quantifying natural language traits such as compositionality \citep{hupkes2020compositionality, dankers2021paradox, chaabouni2020compositionality}, systematic generalization \citep{vani2021iterated, mu2021emergent}, pragmatism \citep{andreas2016reasoning, kang2020incorporating, zaslavsky2020rate}, morphology, and more.

Compositionality is probably the most prominent property of natural language.
Compositionality enables representation of complex meanings using the meaning of parts \cite{li2019ease}.
Thus, a prerequisite for compositionality is the ability to \textbf{decompose} a complex entity to simple parts. In this work, we refer to these simple parts as symbols.

Humans are able to process and use symbols in a variety of ways, which is one of the most interesting aspects of our communication system. 
Quantifying symbolism and compositionality in EC is notoriously difficult \cite{lazaridou2018emergence}.
We defines emergent communication as compositional if: 
1. it is composed from primitive \textit{words} and 
2. each word can be mapped to \textit{symbol} with meaning in some gold language and
3. several words compose a \textit{message} that can be mapped to \textit{phrase} with meaning in the gold language and
4. message can be decomposed back to words

While compositionality is considered a precondition for an emergent language to generalize at scale, recent studies found that common compositionality measures in EC like topographic similarity \cite{brighton2006understanding,lazaridou2018emergence,li2019ease} do not correlate well with success in the task \citep{chaabouni2021emergent, yao2022linking}.


% Topographic similarity (TopSim) is the most common EC evaluation metric.
Topographic similarity estimates the correlation between the distances of all possible pairs of messages and the distances of all possible pair of objects \cite{brighton2006understanding}.
Topographic similarity is a global metric that does not require a reference language and can be easily applied to every EC setup.
However, since this metric does not consider symbols, it cannot directly assess compositionality. 

Recent work \cite{mu2021emergent} suggested to use the adjusted mutual information (AMI) metric \cite{vinh2009information}.
$ AMI\in [0,1]$  measures the mutual information between two clusters, messages and labeling rules adjusted for chance. 
\begin{equation}
\small
\text{AMI}(M, L) = \frac{{I(M, L) - E(I(M, L))}}{{\max(H(M), H(L)) - E(I(M, L))}}
% I(M, L) = \sum_{i=1}^{m} \sum_{j=1}^{l} P(i, j) \log \frac{P(i, j)}{P(i)P^{'}(j)}
\label{eq:ami}
\end{equation}
where $I(M, L)$ is the mutual information between $M$ and $L$, $H(\cdot)$ is the entropy, and $E(I(M, L))$ computes with respect to a hypergeometric model of randomness. %, where M and L represent a set of random permutations, thus are subject to the number of unique values in each cluster.
%, where $P(i, j)$ denotes the probability that a point belongs to cluster $M_i$ in M and cluster $L_j$ in $L$.
% A normalization element is then added to adjust it for chance (see \cite{vinh2009information} for details).
AMI  can be employed as clustering similarity measure.
A higher score indicates overall higher alignment between messages and label phrases.
AMI showed to assess compositionality better than topographic similarity (\cite{mu2021emergent}.

In this work we extend the evaluation framework described by \citeauthor{mu2021emergent} and suggest a finer-grained metric which we refer to as symbol best matching (SBM).
SBM is based on the best-match algorithm \bcr{} from graph theory.
In contrast to other metrics, SBM provides optimal match between EC words and gold language symbols.
Therefore, it directly complies with the compositionality definition mentioned above.
The best match score provides an exact measure for symbolism in the emergent communication.
One can apply the a simple SBM version to object and messages directly.
As such, this metric is highly correlated with AMI.
% SBM advantages become evident when a reference gold language exists with the data.
%Unlike other metrics, SBM requires a reference gold language.
% A gold language is composed from a set of symbols.
Each object in the dataset is described by few symbols from the language.
Communication channel in most ED frameworks allow agents to generate multi-word messages.
Thus one can apply SBM for finding the best match between words and symbols.
Quantifying the best match provides an exact measure for symbolism in the emergent communication.

%==================================================================


%We will use the \Shapes{} game as a running example. 
% Objects in the Shapes{} world are images of shapes.
% There are $ 5 $ unique shapes in the world.
% Each shape has a color. There are 6 unique colors
% \bc{need to continue to describe the game}


==> top_level/chapters/92_related_work.tex <==
\section{Related Work}
\paragraph{Decoding Emergent Communication:}
Communication emerging between artificial agents is not easily interpretable by humans \cite{bennett2021intensional}. 
% As aforementioned, 
Prior work augmented the EC setup with a supervised objective, where the sender classifies objects to natural language labels, while communicating about them \citep{lazaridou2020multi, lowe2020interaction}.
More recent work tried to translate emergent language to human language \cite{yao2022linking, mu2021emergent}. Agents communicate about images, with image captions as target translations. 
They showed that translation quality correlates with transferability to another task better than game accuracy or topographical similarity.
However, in general, one cannot assume that a parallel corpus of emergent messages and corresponding human messages exists, limiting the use of these methods.


\paragraph{Evaluating symbolism}
\label{sec:plan-objective3}
Artificial agents acquire opaque communication protocols that does not clearly resemble human language.
As a result, most efforts focus on characterizing these differences.
Deciphering the emerging protocol may be especially pertinent as artificial agents are increasingly integrated into daily life, and possibly even communicate among themselves.
Specifically, we are interested in assessing the degree to which \emph{symbolic} communication emerges from agents' need to coordinate.

\paragraph{Topographic similarity}
The emergent communication field luck good evaluation metrics. 
The most commonly used evaluation metric is known as Topographic similarity.
Topographic similarity (Ref-41) measure the correlation of the distances between all the possible pairs of meanings and the corresponding pairs of signals.
The intuition behind this measure is that semantically similar objects should have similar messages (thus using ``pair of'')
First compute two lists of numbers: (i) the Levenshtein distances between all pairs of objects’ messages; and (ii) the cosine similarity between all pairs of objects’ VisA vectors. Given these two lists, the topographic similarity is defined as their negative Spearman $\rho$ correlation (since we are correlating distances with similarities, negative values of correlation indicate topographic similarity of the two spaces) (Ref-41).


\paragraph{Topographic Similarity} The topographic similarity \cite{brighton2006understanding, lazaridou2018emergence, yao2022linking} measures how messages align with the object representations. More concretely, let $ cs(\vx_i,\vx_j) = -\vx_i \cdot \vx_j / ||\vx_i||_2 ||\vx_j||_2$
% −Ii · Ij/(||Ii||2||Ij ||2) 
be the negative cosine similarity of objects $\vx_i and \vx_j$, and $ed(m_i, m_j)$ be
the Levenshtein distance \cite{levenshtein1966binary} between messages $m_i$ and $m_j$. The topographic similarity metric is defined as the Spearman rank correlation of the two distance metrics:
\begin{equation}
\begin{split}
    Topsim = \rho(R(ed),R(cs) =\\ \frac{\mathbb{E}_{i,j} [(R(ed_{ij}) − \muR(ed))(R(cs_{ij} ) − \muR(cs))]} {\rhoR(ed)\rhoR(cs)}
\label{eq:top_sim}
\end{split}
\end{equation}
Where $R(\cdot)$ denotes the rank of the element in the list.

\paragraph{Enthropy (H) and AMI}
bc{Ref-55}. 
Information theoretic quantities between the agent messages and concepts:
H(M|C): the conditional entropy of messages given concept
AMI(M,C): the adjusted mutual information
AMI(M,C) = (I(M,C) E(I(M,C))) /(max(H(M), H(C)) E(I(M,C))) (Vinh et al., 2010)


\paragraph{ACR} \citeauthor{mu2021emergent} learns an approximate compositional reconstruction (ACR) by training a model to predict the probability distribution of composed messages given concepts. 


\paragraph{\textbf{Gumbel-softmax}} (GS) is a continuous approximation for a categorical distribution. In the communication context, a discrete message is approximated via a sampling procedure. Details are given elsewhere \cite{havrylov2017emergence_20,jang2016categorical_a2}. 
The GS end result is a continuous message, where each word has the size of the alphabet and holds \emph{one} (approximate) symbol. This allows for end-to-end optimization with gradient methods, and for discrete communication at inference time. However, the channel capacity is limited, and a large alphabet size is both inefficient (due to the need to sample from a large number of categories) and does not perform well in practice.

\paragraph{\textbf{Quantized-communication}} (QT) is discrete approximation to a continuous message. It uses a differentiable rounding approach \cite{carmeli2022emergent} to generate  discrete vectors. In all our experiments we set the scaling factor to $1$ to effectively generate multi-hot vectors in the range $[0, 1]$.
In contrast to GS, QT allows significant channel capacity even at limited word lengths.


==> top_level/chapters/93_methods.tex <==
\section{Methods}
Successfully accomplishing a coordination task is conceived to be a precondition for symbolism and compositionality.
Many game setups have been proposed in the emergent communication literature.
In this work we follow a setup suggested by \cite{mu2021emergent}. 
Formally, we assume a world $\sX$ with $| \sX |$  objects. 
At each turn, $k$, of the game a labeling rule $ l = \{v^i_j\}^n : \sX \mapsto {0, 1} $, explained next, is chosen uniformly at random from a set of rules $\sL$.
Next, $n$ candidate objects $\sX_k = \{x\}^n \subseteq \sX$, are drawn from $\sX$ such that a subset of them, $ \sT_k $, obey to the labeling rule $ l $ and the rest $\sD_k = \sX_k - \sT_k$ are set to be distractors.

At each turn, the sender $S$ encodes the target objects $\sT_k$ via its encoder network $u_\theta$, such that  $u^s = u_\theta(\sT_k) \in \mathbb{R}^{d}$ is the encoded representation of $\sT_k$.
It then uses its channel network $z_\theta$ to generate a, possibly multi-word, message
$m = \{w\}^i= z_\theta(u^s) = z_\theta(u_\theta(\sT_k))$.

At each turn, the receiver $R$ encodes each candidate object $c_i$ ($i=1,\ldots,n$) via its encoder network $u_\phi$, to obtain $u_\phi(c_i)$. 
We write $U^r \in \mathbb{R}^{\sC \times d}$  to refer to the set of encoded candidate representations, each of dimension $d$. 
The receiver then decodes the message via its decoder channel network $z_\phi$, obtaining
$z^r = z_\phi(m) \in \mathbb{R}^d$.
Next, the receiver computes a score matching each of the encoded candidates to the decoded message.
%produces a logits vector $\vg = g(\cdot)$ to decide which of the candidates is the target:
% $g^r(z^r, U^r) \rightarrow \sR^{|\sC|} = \mathrm{softmax}(z^r \cdot U^r)$.
% The receiver then calculates prediction scores $\tilde{\vt_i} =  \mathrm{BCE}(z^r \cdot U^r)$, where BCE is the binary cross entropy function.
The channel and message have certain biases that influence both the communication characteristics and the agents' performance in the game.

Note that in contrast to most referential game setups, here the sender needs to encode multiple targets using a single message.
We hypotheses that for succeeding in the game, sender needs to ``discove'' and communicate some notion of the labeling rule $l$, since the rule is designed to distinguish targets from distractors.
 
% \subsubsection{Successfully Accomplishing a Task}
% While measuring task success is straightforward, assessing the 
% Similar to previous work \citep{kottur2017natural,mordatch2018emergence,resnick2020capacity}, we impose constraints on the communication channel, and examine how they affect the ability to succeed in the task.
% By repeating these across various games and worlds, we can determine which aspects of communication are crucial for coordination to succeed.
% For instance, in our preliminary experiments (Section \ref{sec:preliminary-obj3-noum}) we observed a sweet spot between the possible vocabulary size and the message length.


\subsection{Evaluating Symbolism}
While evaluating game performance is fairly straightforward, evaluating symbolism and compositionality is more involved.
To do so, we focus on datasets for which symbolism can be assessed.
Objects in these datasets have $n$ distinct categorical features $f_1 .. f_n $.
Each feature $ f_i $ has a set of $| v^i | = M^i $ categorical values.
We refer to this $v^i_j$ feature-value pair as FVP.
We further assume an Oracle labeling function $ Oracle(\cdot) :  \rvx  \mapsto \{0, 1\} $ that maps objects to $ v^i_j $ values.
We define a labeling rule $l$ as a Boolean expression over a set of FVPs.
While one may allow $l$ to contain any logical operator, in this work we restrict the Oracle to use just the `AND' $(\land)$ operator.
% \bc{Mu allows not and or as well}.
% Thus, when specifying a labeling rule as $ l = \{v_i^j\}^n $ we refer to a Boolean expression with the AND operator between all operands.
% We further define the identity labeling function $O_{x_i}(\cdot, \cdot): \{\rvx_i, \rvx_j\} \mapsto \{0, 1\} $ that returns $ 1 $ if $\rvx_1 == \rvx_2\ $ and $ 0 $ otherwise.
% We define the label of the data sample labeled by the identity function to be $x_i$.


To summarize, for each data sample   
% $ \{\rvx^s, \rvx^r\} \in \sX_i $ 
$ \{\rvx\}^n \in \sX_k $ in the dataset,
there exist a labeling rule $ l = \{v^i_j\}^m$ such that $ O_l(x) = 1 $ if $ x \in \sT_k  $ and  $ 0 $ otherwise. 
% $\sT_k$ is the set of targets in the sample. 
% With that, we can assume that \FVPs{} is the label of a data sample and search for a mapping $ \gG: m \mapsto l $

%We may take several approaches for searching and defining $ \gG $.
% Specifically, we investigate classification, translations and graph theory which we describe in the following sections.


\subsection{Symbol Best Matching}
Given that both messages and symbols are discrete entities we suggest an evaluation approach that is based on structuring a bipartite graph $\gG$ between them and applying the best-match algorithm \bcr{}.

A bipartite graph $ \gG = (N,  E) $
is a graph where the set of nodes $ N $ can be partitioned into two disjoint sets $ W $ and $ V $ such that every edge in the graph connects a node in $ W $ to a node in $ L $, namely:
\begin{equation}
E \subseteq \{(w, v) \mid w \in W, v \in V\}
\label{eq:graph_construct}
\end{equation}
We construct $\gG $ as follows:
The left-side nodes $ \{w\} $ is the set of unique words generated by the agents for a given dataset.
% Recall that $m = \{w\}^i$ is a multi-word message generated by the agents at each turn of the game.
The right-side nodes $ \{v\} $ is the set of unique FVPs $\{v\}$ assigned by the Oracle $O$ to the dataset.
% Recall that $l = \{v^i_j\}^m $ is a set of values (a.k.a symbols) assigned by the Oracle in each turn of the game.

% for simplifying the discussion we assume that each labeling rule  $l$ is composed from exactly one symbol, namely that $n=1$ and $|{v_i}| = 1 $ and thus can omit the $i$ and $n$ scripts.
Edges in $\gG $ are associated with data samples in the dataset.
Each data sample is associated with a message $m \in M$ generated by the sender, and with a labeling rule $ l \in L$ assigned by the Oracle.
As direct mapping between words $ w \in m$ to symbols $ v^i_j \in l$ is not known, we add the Cartesian multiplication $\{w \times v^i_j\}$ as edges for each data sample. 
We further accumulate all edges with the same left and right nodes into a single edge and assign it a wight $e$ equals to the number of accumulated edges.
See Figure \ref{fig:msg_symbol_graph} for an example and explanation.

\subsubsection{The Best Match Algorithm}
A best match algorithm such as the Hopcroft-Karp \cite{hopcroft1973n}  seeks to find optimal pairing between two set of nodes such that the overall matching score is maximized.
In our context, an optimal match is a one-to-one mapping between words and symbols (FVPs).
\textbf{Such a mapping is fully interpretable and high matching score indicates that agents learn to generate unique word for meaningful symbol.}
Formally, the best-match is a set of edges  $ B \subseteq E $ in a bipartite graph $\gG$ where no two edges in $ B $ share a common node and:
\begin{equation}
Q_{bm} = \arg\max_{B} \sum_{e \in B}q_e
\label{eq:best_match}
\end{equation}

We define $B_{bm}$ to be the $B$ that gain the highest $Q_{bm}$ score. 
Normalizing the best-match assignment by the total number of symbols used by the Oracle to label the dataset resulted in a metric $ 0 < Q_{bm} \leq 1.0 $.
The lower bound of $Q_{bm}$ is equal to $q_{\tilde{e}} / \sum q_i $ where ${\tilde{e}} $ is the edge with the highest weight in $\gG $.

\begin{figure}
\begin{center}
\begin{tikzpicture}
  % Define nodes with colors
  \node[draw, circle, fill=blue!20] (W1) at (0,0) {$w_1$};
  \node[draw, circle, fill=blue!20] (W2) at (0,-1.5) {$w_2$};
  \node[draw, circle, fill=blue!20] (W3) at (0,-3) {$w_3$};
  \node[draw, circle, fill=blue!20] (W4) at (0,-4.5) {$w_4$};

  \node[draw, circle, fill=orange!20] (V1) at (2,0) {$v_1$};
  \node[draw, circle, fill=orange!20] (V2) at (2,-1.5) {$v_2$};
  \node[draw, circle, fill=orange!20] (V3) at (2,-3) {$v_3$};

  % Draw edges with labels and colors
  \draw[color=blue] (W1) -- node[above] {\color{black}10} (V1);
  \draw[color=red] (W1) -- node[above] {\color{black}8} (V2);
  \draw[color=red] (W1) -- node[above=1pt] {\color{black}2} (V3);
  \draw[color=blue] (W2) -- node[above=3pt, xshift=-5pt] {\color{black}3} (V3);
  \draw[color=blue] (W3) -- node[below=3pt, xshift=-5pt] {\color{black}2} (V2);
  \draw[color=mydarkgreen] (W4) -- node[above] {\color{black}2} (V3);
\end{tikzpicture}
\end{center}
\caption{The $ \text{word} \leftrightarrow \text{symbol} $ bipartite graph. Each edge in the graph represents a match between a word and a symbol.
There are three edge types: best match edges (blue), paraphrase edges (green) and ambiguous edges (red).
% The dataset that pertains to the above example consists of 30 samples.
% Each sample in that dataset is labeled with one of three labeling rules, $v_1, v_2, v_3 $.
% There are 10 samples for each symbol.
% Agents generate four unique messages, $ w_1 ... w_4 $ for the $30$ samples such that:
% $|w_1|=23,\, |w_2|=3,\, |w_3|=2\, \text{and}\, |w_4|=2,$.
% We define three edge types: Best match edges (blue), paraphrase edges (green) and ambiguous edges (red).
% The best match set in the above example is composed from 15 edges (samples) and defines the assignment: $\{w_1 \mapsto v_1\}, \{w_2 \mapsto v_3\} \{w_3 \mapsto v_2\}$.
% There are $13$ ambiguous edges, all are $w_1$ messages.
% There are $2$ paraphrase edges. Note that paraphrase edges are belong to messages that are not part of the best match.
% Thus, in for the above example, $Q_{bm}= 15/30=0.5 \quad Q_a = 13/30=0.433 \quad{and} \quad Q_p = 2/30=0.067 $
}
\label{fig:msg_symbol_graph}
\end{figure}

% A random assignment of words to symbols will resulted in a matching score of $ E(Q_{rd}) = |{v}| / \sum(i) $
\subsection{Auxiliary Match Metrics}
We can further assess the bipartite graph by considering edges not in the best match set $ B_{bm} $.
Specifically, two types of edges may exists in $E \setminus B_{bm} $ namely ambiguous $ A $ and paraphrase $ C $ edges.

\paragraph{\textbf{ambiguous edge}} is an edge $ e \in A = \{w, v\} | w \in W_{bm}, v \in V_{bm} $ and $ e \notin B_{bm}$.
In words, an ambiguous edge, $ e \in A $ connects word with a symbol, other than the symbol it is best-matched with.
We refer to such as as 'ambiguous` as it maps the same word to two different symbols.
We thus define the ambiguity metric to be: $ Q_{a} = \sum_{e \in A} q_e$.
% \[ Q_{a} = \sum_{e \in A}({e})\]
Normalizing the ambiguity weight $a$ by the total number of symbols used by the Oracle to label the dataset resulted in a metric $ 0 \leq Q_{a} < 1.0 $.
Note that for the ambiguity metric the lower weight the better.

\paragraph{\textbf{paraphrase edge}} is an edge $ e \in P = \{w, v\} | w \notin W_{bm} $. 
In words, a paraphrase edge, $ e \in P $ connects word-node which is not part of the best match assignment with a symbol-node in the best match set. 
We refer to such edge as as 'paraphrase` as it maps two different words to the same symbols.
We define the ambiguity metric to be: $Q_{p} = \sum_{e \in P}(Q_{e})$
%\[ Q_{p} = \sum_{e \in P}(Q_{e})\]
Normalizing the ambiguity weight $Q_p$ by the total number of symbols used by the Oracle to label a the dataset resulted in a metric $ 0 \leq Q_{a} \leq 1.0 $.
High paraphrasing score, though not negative on its own, implies low level of symbolism.

\subsection{Comparing SBM with AMI}
One may apply the SBM algorithm to match message with labels.
That is, instead of consider words in a multi-word messages as the left-side nodes in $\gG$ we assign the left-side nodes to be the messages themselves.
Similarly, instead of consider symbols in a multi-symbol label $\{v^i_j\}^m, m > 1$ as the right-side nodes in $\gG$ we assign the right-side nodes to be the labels themselves.
Doing so will make SBM and AMI qualitatively similar.
Still, while AMI measures the mutual information between two random variables, relating to the set of messages and set of labels, SBM measure the discrete best match between them.

\subsection{Cartesian addition of edges} Messages and labels can be directly matched, but words and symbols cannot be mapped a-priori.
To overcome this difficulty we add a ``conditinal'' edge from each word in a message to all symbols in a corresponding label. We argue that such addition of conditional edges does not affect the best match score.
Intuitively, assume that for a given best match $B_{bm}$ if an edge $e$ connects a word node $w$ with a symbol node $v_i$ then edges from $w$ to other symbol node $v_j$ does not affect the best match.
To prove, assume by induction on the addition to a graph $\gG$, of: a word node $w$, a label $l$ with a set of symbol nodes $\{v\}^m $ and a set of edges $\{e\}^m$ connecting $w$ to all $\{v\}^m $ nodes.
Consider three cases:
1. If the pair $\{w, v_i\} $ for some $i$ is already in the match then it will remain in the match, as edges are being added to all $v$ nodes.
2. If $w$ is on a match with node other that $v \in \{v\}^m $  and after the addition of $\{e\}^m$, $w$ becomes in match with some $v \in \{v\}^m$ then all other edges from $w$ can be ignored.
2. If $w$ is not on a match with node $v \in \{v\}^m $ even after adding $\{e\}^m$ then all added edges can be ignored.
Importantly, while normalizing the best match score ${bm}$ we take into acount just a single edge for each word $w$. 




